Aligning Text-to-Music Evaluation with Human Preferences

Despite significant recent advances in generative acoustic text-to-music (TTM) modeling, robust evaluation of these models lags behind, relying in particular on the popular Fr\'echet Audio Distance (FAD). In this work, we rigorously study the design space of reference-based divergence metrics for evaluating TTM models through (1) designing four synthetic meta-evaluations to measure sensitivity to particular musical desiderata, and (2) collecting and evaluating on MusicPrefs, the first open-source dataset of human preferences for TTM systems. We find that not only is the standard FAD setup inconsistent on both synthetic and human preference data, but that nearly all existing metrics fail to effectively capture desiderata, and are only weakly correlated with human perception. We propose a new metric, the MAUVE Audio Divergence (MAD), computed on representations from a self-supervised audio embedding model. We find that this metric effectively captures diverse musical desiderata (average rank correlation 0.84 for MAD vs. 0.49 for FAD and also correlates more strongly with MusicPrefs (0.62 vs. 0.14).

==> sections/conclusion.tex <==
\section{Conclusion}

In this work we propose \ourmetric{}, a new evaluation metric for automatic evaluation of TTM models. 
MAD is derived from a systematic meta-evaluation that analyzes the sensitivity of evaluation hyperparameters to various music generation desiderata. 
Specifically, in terms of robustness to variations in other hyperparameters, we find that divergences like \textsc{Mauve} outperform past choices like Fr\'echet Distance, and self-supervised embedding models like MERT outperform discriminative ones. 
We additionally collect and release \textbf{\textit{\ourdata{}}}, 
a first-of-its-kind dataset of pairwise human TTM preferences, 
and use it to demonstrate that \ourmetric{} strongly correlates with human preferences. 
While we do not recommend replacing human evaluations with \ourmetric{}, automatic evaluations can provide a powerful signal for competition and hill-climbing on model performance. We hope \ourmetric{} can provide such a signal for music generation research. 









==> sections/impact.tex <==
\section*{Impact Statement}

The present paper's primary goal is to advance the consistency and robustness of generative TTM evaluation, with the hope of supporting more calibrated benchmarking in the field as a whole. 
While better metrics to evaluate TTM systems necessarily are tied to a number of issues regarding generative music as a whole, such as questions over protecting artists rights and livelihoods, the present research sits orthogonal to these issues, and we hope opens the door for more transparent research into such systems.


==> sections/prefs.tex <==
\section{Collecting \ourdata{}}

Here we describe our approach to collecting a large dataset of human preferences on music generated by state-of-the-art open weights TTM models. 
While analogous resources have driven significant progress in generation for
speech~\cite{somos},
language~\cite{chatbot_arena},
and 
images~\cite{visionprefer}, 
to the best of our knowledge, 
we are the first to collect and release\footnote{Upon publication.} this type of data for TTM. 
This effort involved two high-level steps: 
(1) creating a large dataset of music generated from state-of-the-art open weights TTM models on a set of common text prompts, 
and 
(2) collecting pairwise human preferences on that dataset.

\subsection{Generating Music with Common Prompts} \label{sec:music_data_generation}

\paragraph{Models:} \quad To generate the musical material for \ourdata{}, 
we identify a set of $7$ open weights music generation models that are representative of the current state of the art: 
Stable Audio Open (SAO)~\cite{stable_audio_open}, 
MusicGen small/medium/large~\cite{musicgen}, 
AudioLDM2~\cite{audioldm2}, 
MusicLDM~\cite{musicldm}, and 
Riffusion v1~\cite{riffusion_v1} (the original open weights Riffusion, not the recent commercial model). 
These models vary along notable axes such as 
methodology (codec language models~\cite{vqvae}, latent diffusion models~\cite{ldm}, etc.) 
and 
training data (creative commons music, licensed stock music, etc.). 
We focused on open models both to promote reproducibility and because no commercial model has a %
public 
API. 

\paragraph{Prompts:} \quad We curate a set of $2.6$k prompts which we use as common inputs for all TTM models. 
We limit our prompt set to instrumental only (no vocals)---TTM with vocals usually involves lyrics conditioning, which we leave as an avenue for future work. 
Our prompt set is derived from MusicCaps~\citep{musiccaps_musiclm}, 
a collection of $5.5$k $10$-second YouTube clips with expert-annotated captions. 
Because MusicCaps contains music-to-text \emph{captions} that differ in semantics from text-to-music \emph{prompts}, 
we adopt the prompt set of~\citet{fadtk}, which was created by using ChatGPT~\citep{chatgpt} to rewrite each MusicCaps caption as a prompt. 
We then use ChatGPT to further filter out captions mentioning vocals and others content unexpected for text-to-music-generation (e.g., tutorials and 
everyday 
sounds), 
arriving at a total of $2,617$ text prompts. 
We generate ten outputs from each model for each prompt using distinct random seeds, resulting in $183$k total audio clips.


\subsection{Collecting crowdsourced preferences}


We collect a large dataset of pairwise human preferences via Amazon Mechanical Turk. 
At a high level, users are presented with audio generated by two different systems and asked which of the pair they prefer. 
We collect preferences on $2,520$ output pairs, uniformly distributed across the 21 system pairs, i.e., $120$ preferences per unique pair of system.

\paragraph{Design Decisions:} \quad We make four noteworthy decisions in designing our collection protocol.
Firstly, 
we choose to collect comparative preferences on pairs of models rather than opinion scores on individual models, 
following common practice in evaluation~\citep{schoeffler2015towards}. 
Secondly, 
annotators see pairs of model outputs generated from a common text prompt, 
but we choose to \emph{not} display that prompt to the user. 
Prompts are not an input to divergence metrics---accordingly, we did not want prompt correspondence to bias human annotator preferences. 
Thirdly, we asked annotators to provide an independent preference decision on the basis of fidelity and musicality. 
Fidelity preferences are equal to musicality preferences in $61$\% of pairs. 
Finally, we also allow users to declare a ``tie'' on either axis, so that they are not forced to make a random decision when they cannot meaningfully distinguish---we discard ties. 
See \Cref{fig:annotation_interface} in the appendix for a screenshot of our interface. 


\paragraph{Analysis:} \quad In~\Cref{fig:human_pooled}, 
we visualize the pairwise win rates of individual models vs. other specific models and vs. all others. 
We discard ties from our analysis, which account for $25$\% and $19$\% of preferences for fidelity and musicality respectively. 
We then aggregate preferences together across fidelity and musicality, 
resulting in roughly even weighting for these two axes. 
We observe that the MusicGen family of models compares favorably to all others, 
and that win rates of MusicGen models are correlated with model size. 
We further observe that more broadly the recency of a given model is not strongly correlated with its performance, as the the older MusicGen(s) and MusicLDM perform better than the newest model Stable Audio Open.
See~\Cref{appendix:fullmusicprefs} to see win rates disentangled across musicality and fidelity. 

To measure agreement, we collect preferences from two additional annotators on $126$ pairs selected uniformly at random from \ourdata. 
Annotators reached a true majority in $88$\% of musicality preferences, 
and $76$\% of fidelity preferences.



\input{sections/table_alignment}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{images/pooled.pdf}
    \caption{Each row shows the proportion of instances where one system is preferred over any other individual systems 
    according to the pooled musicality and fidelity judgments. * indicates statistical significance with $P < 0.05$ under the Wilcoxon signed rank test. Note that win rates for opposite sides do not sum to one as we allow ties.}
    \label{fig:human_pooled}
\end{figure}

\section{Measuring Human Preference Alignment} \label{sec:alignment_with_human_preferences}

Given the human feedback data from \ourdata, along with the insight from our synthetic meta-evaluation in designing robust divergences, we can now assess how well our analyzed metrics, including \ourmetric{}, align with human preferences. In particular, we focus here on how the ordering induced by any given divergence metric matches the human rankings from MusicPrefs. We focus on this ranking behavior as the ability to consistently determine the \emph{relative} performance of models (i.e.,~``horse-racing") is integral to modern TTM research in assessing commensurate gains from paper to paper. We compare our proposed \ourmetric{} to the baseline FAD (with both VGGish and CLAP backbones), as well as the induced ranking from the reference-free CLAP-Score metric \cite{clap, clap_score}, which measures control adherence to the underlying text conditions and should be independent of human ranking. 

In Table~\ref{tab:bt_scores}, we show the overall induced rankings by each metric sorted according to the overall human ranking, as well as Kendall's $\tau$ coefficient relative to the overall rankings. Human rankings are calculated through their Bradley-Terry scores, which are linearly equivalent to Elo score and thus more accurately estimate the overall strength of each model than assessing raw win rate \cite{bradley_terry, white, chatbot_arena}.
We find that \ourmetric{} shows a strong and statistically significant correlation with human rankings, nearly exactly matching the human preferences with the exception of a strong preference towards Stable Audio Open. 
In contrast, none of the other metrics correlate in a statistically significant manner.
Note that we do not expect CLAP score to correlate with \ourdata{} as annotators were not shown prompts---we include it here to provide evidence that \ourdata{} measures desiderata orthogonal to control as intended. 















==> sections/preliminaries.tex <==
\section{Preliminaries and Methods}\label{sec:meth}

We study \emph{reference-based} evaluation metrics \citep{naeem2020reliable} that compare the outputs of a generative model to a reference set of representative data from the distribution we intend to model. A reference-based metric quantifies the divergence between the probability distribution of a generative model $q$ and a reference distribution $p$ using a representative sample $\mathbf{x}_{1,\dots,M} \sim p$, i.e., a reference set of $M$ human music performances. To identify salient discrepancies between $q$ and $p$, we define an evaluation metric on features of examples extracted using an \emph{embedding model}. Given $N$ generated audio outputs $\mathbf{y}_{1,\dots,N}$ from a  model $q$, and features $f : \text{audio} \to \mathbb{R}^d$ extracted from an embedding model, a reference-based evaluation metric is a divergence $D(f(\mathbf{y})_{1,\dots,N},f(\mathbf{x})_{1,\dots,M})$  between features of audio generated by $q$ and the reference set.

The design space of reference-based evaluation metrics can therefore be characterized by (1)~the reference distribution $p$ and corresponding reference set, (2)~the embedding model and features $f$ used to process the audio samples, and (3)~the divergence $D$ used to calculate distributional discrepancies in feature space $\mathbb{R}^d$. For example, FAD uses VGGish as an embedding model, activations of the final (pre-classification) VGGish model as features, and the Fréchet distance as a divergence.

\subsection{Choosing a Reference Set}

\citet{fadtk} report that the choice of reference set can heavily influence the performance of automatic metrics and that the commonly used MusicCaps \cite{musiccaps_musiclm} dataset includes a notable amount of low-quality entries and can result in FAD scores poorly correlating with human ratings. In our experiments, we use the FMA-Pop dataset \cite{fadtk}, a curated subset of FMA \cite{fma} emphasizing songs with high play counts under the ``pop'' label. 
FMA-Pop contains $4,230$ songs of $30$ seconds in length each.

\subsection{Extracting Features from Embedding Models}

We study the performance of a variety of audio models as embedding models. In addition to the VGGish model \cite{vggish} originally used for FAD and the higher-performing audio understanding models explored in \citet{fadtk} (CLAP \cite{clap} and MERT \cite{mert}), we experiment with strong music generation models (MusicGen \cite{musicgen} and Jukebox \cite{jukebox}). The motivation to study these self-supervised models as embedding models is that they might more accurately capture salient audio features overlooked by distantly-supervised music  models~\cite{castellon2021codified}.

Given a neural embedding model, we consider several strategies for extracting $d$-dimensional features from this model. A natural candidate for features are internal activations of the model. For a deep neural network with many layers, we must decide which activations to use as features. For audio models, which process temporal data, we must also decide how to aggregate features across time. We study several feature extraction and aggregation strategies in this work. First, we consider features extracted from different layers of the network. Second, we consider four strategies for aggregation across time:
\begin{itemize}
    \item \emph{max-pooling}: the maximum value of each activation across time indices.
    \item \emph{average-pooling}, the mean of activations across time indices.
    \item \emph{last}: activations at the last time index.
    \item \emph{first}: activations at the first time index (only considered for the bi-directional MERT model). 
\end{itemize}
\Cref{tab:emb_models_summary} in Appendix \ref{appendix:full_metaeval} details our search space of embedding backbones, layers, and pooling methods.

\subsection{Calculating Divergences}

We study a variety of divergences for parameterizing an evaluation metric.
The key distinctions between these metrics 
involve how they estimate the reference and generated distributions within the chosen embedding space. FAD \citep{fad} and related metrics use a simplifying assumption that these distributions are Gaussian and calculate the Frechét distance between them. MMD \citep{jayasumana2024rethinking} 
(equivalently referred to as KD or KAD \citep{chung2025kad})
constructs a kernel density estimator of these distributions. The Precision/Recall/Density/Coverage (or PRDC) metrics \citep{naeem2020reliable} use k-NN estimators: Precision/Density/Coverage use k-NN to estimate the support of the reference distribution~$p$ and measure whether the generated samples are supported by~$p$; Recall conversely  uses k-NN to estimate the support of the generative distribution~$q$ and measure whether the reference set is supported by~$q$. \textsc{Mauve} \citep{Mauve_journal} uses k-means to form discrete histogram estimates of $p$ and $q$, and calculates information divergences between these discrete approximations. Among the metrics we study, \textsc{Mauve} and Recall are the only metrics that form an estimate of the generated distribution $q$ that is more expressive than a single Gaussian (FAD) but less open than pairwise kernel similarity (MMD).


 



==> sections/related.tex <==
\section{Related Work}

Generative music systems, and in particular \emph{audio-domain} systems, have seen a renaissance in recent years driven by the wider methodological explosion in generative models, owing core advances to technical insights from language models  \citep{jukebox, musicgen} and diffusion models \citep{musicldm, stable_audio_open, audioldm2, riffusion_v1}.
Despite many technical similarities with the text and image domains, the space of work on generative evaluation is much less developed for TTM. 
While \citet{fad} and \citet{fadtk} have attempted to assess the quality of evaluation metrics in TTM systems (which has led to better FAD backbones being adopted in further research \citep{Novack2024Ditto, Novack2024Ditto2, Ciranni2024COCOLACC}), these \emph{only} considered Frechét Distance as a metric, and only considered fidelity distortions in their analyses.
While some TTM works have included additional metrics outside FAD and the reference-free CLAP score \citep{nistal2024diff, Novack2025Presto, musicldm, saito2024soundctm, stable_audio_open}, such works purely rely on the assumption that insights from the image modality \citep{jayasumana2024rethinking, naeem2020reliable} would transfer to TTM, with no empirical verification. 
\citet{audiogen_meta_eval} and \citet{chung2025kad} are perhaps the most similar to the present work, with the former focusing on benchmarking evaluation metrics for older audio synthesis models (with no strong correlation found with human perception), and the latter exploring the MMD metric used in earlier TTM works \citep{Novack2025Presto, nistal2024diff, nistal2024improving} for foley generation.












